Towards Fast Computation of Certified Robustness for ReLU Networks

Verifying the robustness property of a general Rectified Linear Unit (ReLU) network is an NP-complete problem [Katz, Barrett, Dill, Julian and Kochenderfer CAV17]. Although finding the exact minimum adversarial distortion is hard, giving a certified lower bound of the minimum distortion is possible. Current available methods of computing such a bound are either time-consuming or delivering low quality bounds that are too loose to be useful. In this paper, we exploit the special structure of ReLU networks and provide two computationally efficient algorithms Fast-Lin and Fast-Lip that are able to certify non-trivial lower bounds of minimum distortions, by bounding the ReLU units with appropriate linear functions Fast-Lin, or by bounding the local Lipschitz constant Fast-Lip. Experiments show that (1) our proposed methods deliver bounds close to (the gap is 2-3X) exact minimum distortion found by Reluplex in small MNIST networks while our algorithms are more than 10,000 times faster; (2) our methods deliver similar quality of bounds (the gap is within 35% and usually around 10%; sometimes our bounds are even better) for larger networks compared to the methods based on solving linear programming problems but our algorithms are 33-14,000 times faster; (3) our method is capable of solving large MNIST and CIFAR networks up to 7 layers with more than 10,000 neurons within tens of seconds on a single CPU core. In addition, we show that, in fact, there is no polynomial time algorithm that can approximately find the minimum $\ell_1$ adversarial distortion of a ReLU network with a $0.99\ln n$ approximation ratio unless $\mathsf{NP}$=$\mathsf{P}$, where $n$ is the number of neurons in the network.

==> _app_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Comparison of our proposed certified lower bounds \textbf{Fast-Lin} and \textbf{Fast-Lip}, the lower bounds found by \textbf{LP} and \textbf{LP-Full}, the lower bounds found by \textbf{Clever}, the exact minimum distortion found by \textbf{Reluplex}, and the upper bounds found by \textbf{Attack} algorithms (PGD for $p = \infty$, CW for $p = 2$, EAD for $p = 1$) on 2, 3 layers small MNIST networks with 20 nodes.}
\label{tab:tab1-smallnetwork}
\scalebox{0.65}{
\begin{tabular}{|c|c|c|cccc||c||cc|cccc||c||cc|}
\hline
\multicolumn{3}{|c|}{Small Networks}                                                                                                 & \multicolumn{7}{c|}{Average Magnitude of Distortion on 100 Images}                           & \multicolumn{7}{c|}{Running Time per Image}                                              \\ \hline
\multirow{2}{*}{Network}                                                    & \multirow{2}{*}{$p$-norm}   & \multirow{2}{*}{Target}  & \multicolumn{4}{c||}{Certified Bounds}    & \multicolumn{1}{c||}{Exact}  & \multicolumn{2}{c|}{Uncertified}      & \multicolumn{4}{c||}{Certified Bounds}   & \multicolumn{1}{c||}{Exact}  & \multicolumn{2}{c|}{Uncertified}    \\ \cline{4-17}
                                                                            &                             &                          & Fast-Lin & Fast-Lip & LP        & LP-Full & Reluplex                     & Clever & Attack                       & Fast-Lin & Fast-Lip & LP       & LP-Full & Reluplex                     & Speedup & Attack                    \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ 2*{[}20{]}\end{tabular}} & \multirow{3}{*}{$p=\infty$} & top2                     & 0.01904  & 0.01667  & 0.01968   & 0.01968 & 0.04145                      &        & 0.08538                      &  3 ms    &  4 ms    & 38 ms    &  2 s    &  134 s                       &         & 34 ms                     \\
                                                                            &                             & rand                     & 0.03073  & 0.02699  & 0.03189   & 0.03189 & 0.07765                      &        & 0.15713                      &  3 ms    &  6 ms    & 42 ms    &  2 s    &  38 s                        &         & 34 ms                     \\
                                                                            &                             & least                    & 0.04455  & 0.03976  & 0.04618   & 0.04618 & 0.11711                      &        & 0.19533                      &  3 ms    &  10 ms   & 45 ms    &  2 s    &  360 s                       &         & 34 ms                     \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=2$}      & top2                     & 0.03708  & 0.21944  & 0.04204   & 0.56372 & -                            &        & 0.64669                      &  3 ms    &  33 ms   &  2 s     &  21 s   &  -                           &         & 381 ms                    \\
                                                                            &                             & rand                     & 0.05251  & 0.37414  & 0.05937   & 0.91816 & -                            &        & 1.19630                      &  3 ms    &  43 ms   &  2 s     &  23 s   &  -                           &         & 381 ms                    \\
                                                                            &                             & least                    & 0.07418  & 0.60673  & 0.08653   & 1.34214 & -                            &        & 1.88830                      &  3 ms    &  51 ms   &  4 s     &  26 s   &  -                           &         & 381 ms                    \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=1$}      & top2                     & 0.03832  & 2.11064  & 0.04322   & 2.81713 & -                            &        & 5.38380                      &  3 ms    &  62 ms   &  2 s     &  16 s   &  -                           &         & 342 ms                    \\
                                                                            &                             & rand                     & 0.05387  & 3.84835  & 0.06075   & 4.68225 & -                            &        &11.47600                      &  3 ms    &  73 ms   &  2 s     &  17 s   &  -                           &         & 342 ms                    \\
                                                                            &                             & least                    & 0.07598  & 6.35152  & 0.08869   & 6.83578 & -                            &        &19.59600                      &  3 ms    &  82 ms   &  2 s     &  18 s   &  -                           &         & 342 ms                    \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ 3*{[}20{]}\end{tabular}} & \multirow{3}{*}{$p=\infty$} & top2                     & 0.01582  & 0.00938  & 0.01680   & 0.17070 & 0.04234                      &        & 0.12832                      &  5 ms    &   5 ms   &  478 ms  &  6 s    &  4.7 hrs                     &         & 35 ms                     \\
                                                                            &                             & rand                     & 0.02286  & 0.01422  & 0.02414   & 0.02462 & 0.06824                      &        & 0.15867                      &  6 ms    &   7 ms   &  564 ms  &  7 s    &  11.6 hrs                    &         & 35 ms                     \\
                                                                            &                             & least                    & 0.03029  & 0.01957  & 0.03194   & 0.03264 & 0.10449                      &        & 0.26716                      &  5 ms    &   9 ms   &  585 ms  &  7 s    &  12.6 hrs                    &         & 35 ms                     \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=2$}      & top2                     & 0.03510  & 0.08422  & 0.03906   & 0.49015 & -                            &        & 0.74117                      &  6 ms    &  43 ms   &  2 s     &  57 s   &  -                           &         & 382 ms                    \\
                                                                            &                             & rand                     & 0.04470  & 0.12876  & 0.04906   & 0.70955 & -                            &        & 1.22570                      &  5 ms    &  58 ms   &  2 s     &  66 s   &  -                           &         & 382 ms                    \\
                                                                            &                             & least                    & 0.05642  & 0.18975  & 0.06247   & 0.94241 & -                            &        & 1.71090                      &  5 ms    &  70 ms   &  2 s     &  77 s   &  -                           &         & 382 ms                    \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=1$}      & top2                     & 0.03653  & 0.65567  & 0.04051   & 2.50097 & -                            &        & 6.13750                      &  5 ms    & 107 ms   &  3 s     &  75 s   &  -                           &         & 318 ms                    \\
                                                                            &                             & rand                     & 0.04618  & 1.18553  & 0.05057   & 3.57400 & -                            &        &10.72200                      &  5 ms    & 129 ms   &  3 s     &  82 s   &  -                           &         & 318 ms                    \\
                                                                            &                             & least                    & 0.05822  & 1.99773  & 0.06431   & 4.69673 & -                            &        &15.68500                      &  5 ms    & 145 ms   &  3 s     &  86 s   &  -                           &         & 318 ms                    \\ \hline
\end{tabular}
}
\end{table*}


==> _notuse_tab_notation.tex <==

 \begin{table*}[!t]
   \caption{Table of Notation\label{tab:notation}}
    \centering
  \scalebox{0.9}
  {
  \begin{tabular}{l l|l l}
      \hline
\!\!Notation  &  \!\!\!Definition & \!\!Notation  & \!\!\!Definition\\ \hline
\!\!$d$ & \!\!\!dimensionality of the input vector\!\! &\!\!$\Delta_{p,\text{min}}$ & \!\!\!minimum $\ell_p$ distortion of $\bm{x_0}$\\
\!\!$K$ & \!\!\!number of output classes &\!\!$\beta_L$&\!\!\!lower bound of minimum distortion\!\!\\
\!\!$f: \R^d \rightarrow \R^K$ & \!\!\!neural network classifier &\!\!$\beta_U$&\!\!\!upper bound of minimum distortion\!\!\\
\!\!$\bm{x_0}\in \R^d$ & \!\!\!original input vector &\!\!$L_q^j$&\!\!\!Lipschitz constant \\
\!\!$\bm{x_a}\in \R^d$ & \!\!\!adversarial example &\!\!$L_{q,x_0}^{j}$ & \!\!\!local Lipschitz constant\\
\!\!$\bm{\delta} \in \R^d$ & \!\!\!distortion$\ :=\bm{x_a}-\bm{x_0}$ &\!\!$B_p(\bm{x_0},R)$&\!\!\!hyper-ball with center $\bm{x_0}$ and radius $R$\!\!\\
\!\!$\|\bm{\delta}\|_p$ & \!\!\!$\ell_p$ norm of distortion, $p \geq 1$\!\! & \!\!CDF&\!\!\!cumulative distribution function\\
\hline
  \end{tabular}
  }
\end{table*}

==> _theory_earlier_nouse.tex <==
There are some verification techniques available in discussing the properties of ReLU networks \textcolor{red}{[reluplex]}. In the following, we study the robustness guarantee of neural networks when the activation function is ReLU.  

\section{The Lipschitz constant of ReLU activation}
\subsection{2-layer NN}

\subsubsection*{Global bound}
The $j_{\text{th}}$ output of a one-hidden-layer neural network can be written as 
\begin{equation*}
	f_j(\bm{x}) = \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \sum_{i=1}^{d} \bm{W}_{ri} \cdot x_i + b_r \right ) = \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ), 
\end{equation*}
where $\sigma (z) = \max (z, 0)$ is ReLU activation function, $\bm{W}$ and $\bm{V}$ are the weight matrices of the first and second layer respectively, and $\bm{w}_r$ is the $r_{\text{th}}$ row of $\bm{W}$. Thus, we can compute $g(\bm{x})$ and $\| \nabla g(\bm{x}) \|_q$ below: 
\begin{align*}
g(\bm{x}) = f_c(\bm{x}) - f_j(\bm{x})
          &= \sum_{r=1}^{U} \bm{V}_{cr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) -  \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) \\
          &= \sum_{r=1}^{U} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) 
\end{align*}
and
\begin{align*}
\| \nabla g(\bm{x}) \|_q &= \left \| \sum_{r=1}^{U} \mathbb{I}(\bm{w}_r \bm{x} + b_r) ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \right \|_q,
\end{align*}
where $\mathbb{I}(z)$ is an univariate indicator function:
\[
\mathbb{I}(z) = \Big \{
  \begin{tabular}{cc}
  1, & \text{if $z>0$,} \\
  0, & \text{if $z \leq 0$.}
  \end{tabular}
\]
We can also rewrite $g(\bm{x})$ and $\| \nabla g(\bm{x}) \|_q$ as 
\begin{align*}
g(\bm{x}) &= \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot (\bm{w}_r \bm{x} + b_r), \\
\| \nabla g(\bm{x}) \|_q &=  \| \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q ,
\end{align*}
where $A(\bm{x})$ is an index set of activated nodes, i.e  $A(\bm{x}) := \{r \mid \bm{w}_r \bm{x} + b_r > 0 \}$. A global upper bound of $\| \nabla g(\bm{x}) \|_q$ can be computed as follows:
\begin{align}
\| \nabla g(\bm{x}) \|_q &=  \| \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q  \label{eq:exact_grad_g} \\  \nonumber
						&\leq \sum_{r \in A(\bm{x})} \| ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q \\ \nonumber
                        &= \sum_{r \in A(\bm{x})} |\bm{V}_{cr} - \bm{V}_{jr}| \cdot \| \bm{w}_r^\top \|_q \\ 
                        &\leq \sum_{r=1}^{d} |\bm{V}_{cr} - \bm{V}_{jr}| \cdot \| \bm{w}_r^\top \|_q. \label{eq:global_bnd_grad_g}
\end{align}
Therefore, we can actually obtain a global upper bound of the Lipschitz constant $L_q$ by evaluating \eqref{eq:global_bnd_grad_g} and don't have to do sampling. 

\subsubsection*{Tighten the bound of $L_{q,x_0}$}
In fact, if we can find out all possible $A(\bm{x})$ around $\bm{x}_0$, e.g. looking at the fixed ball $B_p(\bm{x}_0,R)$ and its corresponding $A(\bm{x})$, then we can obtain the exact value of $L_q$ by computing \eqref{eq:exact_grad_g}. This can be possibly realized in several ways: 
\begin{enumerate}
\item[(a)] via sampling on the $B_p(\bm{x}_0,R)$
\item[(b)] construct the neighborhood geometry by computing the distance to the hyperplanes.
\item[(c)] via constructing bounds on the activation status (will be discussed in the next section)
\end{enumerate}


\section{Some Results on 3-layer NN \textcolor{red}{WIP}}

Given $u \in \R^t$, $v\in \R^{k \times t}$, $w\in \R^{d \times k}$, where $u_j \in \R$ is the $j$-th coordinate of $u$, $v_{j,i} \in \R$ is the $j,i$-th entry of $v$, and $w_i \in \R^d$ is the $i$-th column vector of $w$.
Suppose we are using a general activation function $\phi$.

\begin{align*}
f(x) = \sum_{j=1}^t u_j \cdot \phi \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right)
\end{align*}

We can compute the first derivative
\begin{align*}
\frac{\partial f(x)}{\partial x} = & \left[ \sum_{j=1}^t u_j \cdot \phi' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right) \right. \\
& ~ \left. \sum_{i=1}^k v_{j,i} \phi'(w_i^\top \cdot x) w_i   \right]
\end{align*}

For ReLU, the activation depends on the sign of both $w_i^\top \cdot x$ and $\sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x)$ (ignoring a bias). A global bound can be given, but will be even weaker than~\eqref{eq:global_bnd_grad_g} (roughly up to a factor of $\sum_{j=1}^t | u_j |$).

and compute the second derivative (For ReLU, the second derivative is 0)
\begin{align*}
\frac{\partial^2 f(x)}{ \partial x^2 } = & ~ \left[ \sum_{j=1}^t u_j \cdot \phi'' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right) \right. \\
& ~ \cdot \sum_{i=1}^k v_{j,i} \phi'(w_i^\top \cdot x) \sum_{i'=1}^k v_{j,i'} \phi'(w_{i'}^\top x) w_i w_{i'}^\top  \\
& ~ + \sum_{j=1}^t u_j \cdot \phi' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right)  \\
& ~ \left. \cdot \sum_{i=1}^k v_{j,i} \phi''(w_i^\top \cdot x) w_i w_i^\top   \right]
\end{align*}

\section{Sufficient condition on activation not change}

\subsection{2-layer NN}
Without loss of generality, let's look at the 1st unit (node) in the hidden layer. If $x+\delta$ has the same activation as $x$, it means that either they are both activated  
\begin{align}
	& \sum_{i=1}^{d} W_{1i} x_i + b_1 > 0 \\ 
    & \sum_{i=1}^{d} W_{1i} (x_i+\delta_i) + b_1 > 0 
\end{align}
or they are both deactivated
\begin{align}
	& \sum_{i=1}^{d} W_{1i} x_i + b_1 \leq 0 \\ 
    & \sum_{i=1}^{d} W_{1i} (x_i+\delta_i) + b_1 \leq 0. 
\end{align}
If $\delta$ satisfies the following condition, then the activation status will not change (i.e. the sufficient condition of remaining the same activation status):
\begin{equation}
 	| \sum_{i=1}^{d} W_{1i} \delta_i | < |\sum_{i=1}^{d} W_{1i} x_i + b_1 |. 
\end{equation}
Meanwhile, with H\"older's inequality, we can bound $| \sum_{i=1}^{d} W_{1i} \delta_i |$ as follows 

\begin{equation}
	| \sum_{i=1}^{d} W_{1i} \delta_i | \leq \| W_{1:} \|_q \cdot \| \delta \|_{p} , 
\end{equation}
where $1/p + 1/q = 1$, $p,q \geq 1$. Therefore, if we have 
\begin{equation}
\| W_{1:} \|_q \cdot \| \delta \|_{p} < |\sum_{i=1}^{d} W_{1i} x_i + b_1 | \Rightarrow  \| \delta \|_{p} < \frac{|\sum_{i=1}^{d} W_{1i} x_i + b_1|}{\| W_{1:} \|_q},
\end{equation}
then we can make sure $x$ and $x+\delta$ have the same activation status on the node 1 in the hidden layer. Similarly, we can derive the sufficient condition for node $j$ and the sufficient condition for all the nodes remaining the same activation status is 
\begin{equation}
\label{eq:sufficient_delta_same_act}
	\| \delta \|_{p} \leq \inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q}. 
\end{equation}

\section{Combine LP formulation with activation status}
\begin{eqnarray}
\underset{\delta}{\text{minimize  }} && \| \delta \|_p \nonumber\\
\text{subject to } && g(x_0 + \delta) < 0 \label{eq:general_opt}
\end{eqnarray}
where $g(x_0 + \delta) = f_c(x_0 + \delta) - f_j(x_0 + \delta)$ and $f(x_0 + \delta) = W^{(n)} \sigma(W^{(n-1)} \sigma(...W^{(1)}(x_0 + \delta)))$, where $W^{(n)}$ is the weight matrix of $n$th layer. The optimization formulation is exact -- if we can solve \eqref{eq:general_opt}, we get an effective attack with minimal norm. However, the constraint set in \eqref{eq:general_opt} is non-convex for general activation function.  For ReLU, the constraint set can be non-convex as well. Below, we discuss the cases where the constraint set is linear in 2-layer NN. 

\subsection{2-layer NN}
If we add the bound \eqref{eq:sufficient_delta_same_act} as an additional constraint in \eqref{eq:general_opt}, then we are guaranteed that the activation status won't change for $x_0 + \delta$ and we can directly solve the following without using the constraints in Bastani's paper:
\begin{eqnarray}
\underset{\delta}{\text{minimize  }} && \| \delta \|_p \nonumber\\
\text{subject to } &&  \sum_{r \in A(\bm{x_0})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot (\bm{w}_r (\bm{x}_0+\bm{\delta}) + b_r) < 0 \label{eq:lily_bastani_opt} \\
&&  \| \delta \|_{p} \leq \inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q} \nonumber 
\end{eqnarray}
If \eqref{eq:lily_bastani_opt} is feasible, then $\delta^*$ is the minimum distortion of $\bm{x}_0$ and we should get the same solution as Bastani's paper; if \eqref{eq:lily_bastani_opt} is infeasible, then $\inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q}$ is a strict lower bound of minimum distortion (i.e. we won't over-approximate the lower bound as in the calculation in clever).   

Alternatively, we can also combine the idea of Lipschitz constant with the activation status and obtain a strict analytic lower bound for $\bm{x}_0$ (to be illustrated later)


%% Previous draft of discussing activation status
\textcolor{red}{Previous draft}


\subsection{Upper bounds of $\Lipsloc$}
Suppose there are $N$ possible activation patterns $\{ \set{S}^{(1)}, \ldots, \set{S}^{(N)}  \}$, where $\set{S}^{(i)} = \prod_{k=1}^{M-1}\setA_k(\x^{(i)})$ with $\x^{(i)} \in B_p(\xo,R)$, and let $\set{V} = \bigcap_{i=1}^{N} \set{S}^{(i)}, \set{U} = \bigcup_{i=1}^{N} \set{S}^{(i)}$. The Lipschitz constant can be upper bounded by:
\begin{align}
  & \max_{\x \in B_p(\xo,R)} \| \nabla g_j(\x) \|  \notag \\
 =& \max_{\{ \set{S}^{(1)}, \ldots , \set{S}^{(N)}  \}} \| \nabla g_j(\x) \| \notag \\
 =& \max_{r=1 \in [N] } \left\| \sum_{[i_k]_{k=1}^{M-1} \in \set{V} \cup (\set{S}^{(r)} \setminus \set{V}) } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \right\| \notag \\
 \leq & \quad \left\| \sum_{[i_k]_{k=1}^{M-1} \in \set{V} } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \right\| \notag \\ 
 &+ \max_{r \in [N] } \left\| \sum_{[i_k]_{k=1}^{M-1} \in  \set{S}^{(r)} \setminus \set{V} } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \right\|  \notag \\ 
 \leq & \quad \left\| \sum_{[i_k]_{k=1}^{M-1} \in \set{V} } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \right\| \notag \\ 
 &+ \max_{r \in [N] } \sum_{[i_k]_{k=1}^{M-1} \in \set{S}^{(r)} \setminus \set{V}} \| \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \| \notag \\
 \leq & \quad \left\| \sum_{[i_k]_{k=1}^{M-1} \in \set{V} } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \right\| \notag \\ 
 &+ \sum_{[i_k]_{k=1}^{M-1} \in \set{U} \setminus \set{V}} \| \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top \| \notag 
\end{align}

Given the input constraint $\| \x-\xo \|_p \leq R$, we can propagate it layer by layer and check the activation status of neurons in each layer. For neuron $i$ in layer $k$, there are four possible status:
\begin{itemize}
\item[(a)] the neuron is always activated
	\begin{itemize}
	\item[i.e] $\forall \x \in B_p(\xo,R), \z_i^{(k)}(\x) =  \z_i^{(k)}(\x_0) = 1$ 
	\end{itemize}
\item[(b)] the neuron could change from activated to inactivated
	\begin{itemize}
	\item[i.e] $\exists \x \in B_p(\xo,R), \z_i^{(k)}(\x) = 0, \z_i^{(k)}(\x_0) = 1$ 
	\end{itemize}
\item[(c)] the neuron could change from inactivated to activated
	\begin{itemize}
	\item[i.e] $\exists \x \in B_p(\xo,R), \z_i^{(k)}(\x) = 1, \z_i^{(k)}(\x_0) = 0$ 
	\end{itemize}
\item[(d)] the neuron is always inactivated
	\begin{itemize}
	\item[i.e] $\forall \x \in B_p(\xo,R), \z_i^{(k)}(\x) =  \z_i^{(k)}(\x_0) = 0$ 
	\end{itemize}
\end{itemize}
The $\set{V}$ defined above is in fact the set of indices of neurons satisfying (a), whereas $\set{U}$ is the set of indices of all neurons satisfying (a) or (b) or (c). Note that neurons in (d) are never activated and thus do not belong to $\set{S}^{(r)}$.

% =& \max_{r=1,\ldots,N} \| \sum_{[i_k]_{k=1}^{M-1} \in \set{S}^{(r)} } \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W^{(1)}(i_1,:)^\top \| \\

\subsection{Find out all possible activation patterns}
\textcolor{blue}{Describe how to propagate the constraint $\| \x-\xo \|_p \leq R$ to find out the output range of each neuron}


\textcolor{red}{Previous draft}



\subsection{Lipschitz constant of ReLU network} 
Let $\setA_k(\x) = \{i \mid \z_i^{(k)}(\x) = 1 \}$ denotes the set of activated neurons in layer $k$ with $\z_i^{(k)}(\x)$ being the indicator variable of activation status for neuron $i$ in layer $k$:
\begin{equation*}
  \z_i^{(k)}(\x) =
  \begin{cases}
    1 & \text{if $\W{(k)}\phi_{k-1}(\x)+\bias{(k)} > 0$, (activated)} \\
    0 & \text{otherwise, (inactivated)}
  \end{cases}
\end{equation*}
we show that the gradient of $i_M$th output in a ReLU network, $f_{i_M}(\x) = [\phi_M(\x)]_{i_M}$, is only dependent on the weights of activated neurons:
\begin{equation}
\label{eq:grad_Mlayer}
\nabla f_{i_M}(\x) = \sum_{[i_k]_{k=1}^{M-1} \in \prod_{k=1}^{M-1}\setA_k(\x)} \beta_{i_{1}, \cdots, i_{M-1}}^{(i_M)} \W{(1)}(i_1,:)^\top
\end{equation}
where 
\begin{equation*}
	\beta_{i_{1}, \cdots, i_{M-1}}^{(i_M)} := \prod_{k=1}^{M-1} \W{(k+1)}(i_{k+1},i_k),
\end{equation*}
$\W{}(i,j)$ is the $(i,j)$th entry of matrix $\W{}$, \mbox{$\W{}(i,:)$} is the $i$th row of matrix $\W{}$, $[i_k]_{k=1}^{T}$ is a shorthand for the $T$-tuple $(i_1,i_2,\cdots,i_T)$ and $\prod_{k=1}^{T}\setA_k(\x)$ is a shorthand for the Cartesian product $\setA_1(\x)\times \cdots \times \setA_{T}(\x) = \{(i_1,i_2,\cdots,i_T) \mid i_k \in \setA_k, \forall k \in [T]\}$.


The local Lipschitz constant $\Lipsloc$ of $g_j(\x) = f_c(\x)-f_j(\x)$ is the maximum norm of $\nabla g_j(\x)$ where $\x \in B_p(\xo,R)$. With \eqref{eq:grad_Mlayer}, $\nabla g_j(\x)$ for a $M$-layer ReLU network can be calculated as 
\begin{equation*}
	\nabla g_j(\x) = \sum_{[i_k]_{k=1}^{M-1} \in \prod_{k=1}^{M-1}\setA_k(\x)} \alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} \W{(1)}(i_1,:)^\top  
\end{equation*}
where
\begin{equation*}
	\alpha_{i_{1}, \cdots, i_{M-1}}^{(c,j)} := \beta_{i_{1}, \cdots, i_{M-1}}^{(c)} - \beta_{i_{1}, \cdots, i_{M-1}}^{(j)}.
\end{equation*}\textcolor{blue}{Hongge: Note that since gradient only depends on local information we can assume the sets of activated neurons do not change.}
Notice that $\nabla g_j(\x)$ only depends on the activation patterns $\prod_{k=1}^{T}\setA_k(\x)$ and that the number of activation patterns is finite. Thus, given an example $\xo$, if we enumerate all the possible activation patterns within the ball $B_p(\xo,R)$, we can get the exact local Lipschitz constant $\Lipsloc$ which is the maximum value of $\| \nabla g_j(\x) \|$. However, the number of all possible patterns grows exponentially as the number of activated neurons increases. In this paper, we aim at finding an approximate upper bound for $\| \nabla g_j(\x) \|$, which gives us an upper bound for $\Lipsloc$ and therefore guarantees a \textit{strict} lower bound on the minimum distortion. 


In other words, for the inputs having the same activation patterns (i.e. $\x \neq \x', \setA_k(\x) = \setA_k(\x'), k = 1, \ldots, M$), the gradient vectors are the same, $\nabla f_{i_M}(\x) = \nabla f_{i_M}(\x')$.

\section{The Lipschitz constant of ReLU activation}
\subsection{2-layer NN}

\subsubsection*{Global bound}
The $j_{\text{th}}$ output of a one-hidden-layer neural network can be written as 
\begin{equation*}
	f_j(\bm{x}) = \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \sum_{i=1}^{d} \bm{W}_{ri} \cdot x_i + b_r \right ) = \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ), 
\end{equation*}
where $\sigma (z) = \max (z, 0)$ is ReLU activation function, $\bm{W}$ and $\bm{V}$ are the weight matrices of the first and second layer respectively, and $\bm{w}_r$ is the $r_{\text{th}}$ row of $\bm{W}$. Thus, we can compute $g(\bm{x})$ and $\| \nabla g(\bm{x}) \|_q$ below: 
\begin{align*}
g(\bm{x}) = f_c(\bm{x}) - f_j(\bm{x})
          &= \sum_{r=1}^{U} \bm{V}_{cr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) -  \sum_{r=1}^{U} \bm{V}_{jr} \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) \\
          &= \sum_{r=1}^{U} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot \sigma \left ( \bm{w}_r \bm{x} + b_r \right ) 
\end{align*}
and
\begin{align*}
\| \nabla g(\bm{x}) \|_q &= \left \| \sum_{r=1}^{U} \mathbb{I}(\bm{w}_r \bm{x} + b_r) ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \right \|_q,
\end{align*}
where $\mathbb{I}(z)$ is an univariate indicator function:
\[
\mathbb{I}(z) = \Big \{
  \begin{tabular}{cc}
  1, & \text{if $z>0$,} \\
  0, & \text{if $z \leq 0$.}
  \end{tabular}
\]
We can also rewrite $g(\bm{x})$ and $\| \nabla g(\bm{x}) \|_q$ as 
\begin{align*}
g(\bm{x}) &= \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot (\bm{w}_r \bm{x} + b_r), \\
\| \nabla g(\bm{x}) \|_q &=  \| \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q ,
\end{align*}
where $A(\bm{x})$ is an index set of activated nodes, i.e  $A(\bm{x}) := \{r \mid \bm{w}_r \bm{x} + b_r > 0 \}$. A global upper bound of $\| \nabla g(\bm{x}) \|_q$ can be computed as follows:
\begin{align}
\| \nabla g(\bm{x}) \|_q &=  \| \sum_{r \in A(\bm{x})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q  \label{eq:exact_grad_g} \\  \nonumber
						&\leq \sum_{r \in A(\bm{x})} \| ( \bm{V}_{cr} - \bm{V}_{jr} ) \bm{w}_r^\top \|_q \\ \nonumber
                        &= \sum_{r \in A(\bm{x})} |\bm{V}_{cr} - \bm{V}_{jr}| \cdot \| \bm{w}_r^\top \|_q \\ 
                        &\leq \sum_{r=1}^{d} |\bm{V}_{cr} - \bm{V}_{jr}| \cdot \| \bm{w}_r^\top \|_q. \label{eq:global_bnd_grad_g}
\end{align}
Therefore, we can actually obtain a global upper bound of the Lipschitz constant $L_q$ by evaluating \eqref{eq:global_bnd_grad_g} and don't have to do sampling. 

\subsubsection*{Tighten the bound of $L_{q,x_0}$}
In fact, if we can find out all possible $A(\bm{x})$ around $\bm{x}_0$, e.g. looking at the fixed ball $B_p(\bm{x}_0,R)$ and its corresponding $A(\bm{x})$, then we can obtain the exact value of $L_q$ by computing \eqref{eq:exact_grad_g}. This can be possibly realized in several ways: 
\begin{enumerate}
\item[(a)] via sampling on the $B_p(\bm{x}_0,R)$
\item[(b)] construct the neighborhood geometry by computing the distance to the hyperplanes.
\item[(c)] via constructing bounds on the activation status (will be discussed in the next section)
\end{enumerate}


\section{Some Results on 3-layer NN \textcolor{red}{WIP}}

Given $u \in \R^t$, $v\in \R^{k \times t}$, $w\in \R^{d \times k}$, where $u_j \in \R$ is the $j$-th coordinate of $u$, $v_{j,i} \in \R$ is the $j,i$-th entry of $v$, and $w_i \in \R^d$ is the $i$-th column vector of $w$.
Suppose we are using a general activation function $\phi$.

\begin{align*}
f(x) = \sum_{j=1}^t u_j \cdot \phi \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right)
\end{align*}

We can compute the first derivative
\begin{align*}
\frac{\partial f(x)}{\partial x} = & \left[ \sum_{j=1}^t u_j \cdot \phi' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right) \right. \\
& ~ \left. \sum_{i=1}^k v_{j,i} \phi'(w_i^\top \cdot x) w_i   \right]
\end{align*}

For ReLU, the activation depends on the sign of both $w_i^\top \cdot x$ and $\sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x)$ (ignoring a bias). A global bound can be given, but will be even weaker than~\eqref{eq:global_bnd_grad_g} (roughly up to a factor of $\sum_{j=1}^t | u_j |$).

and compute the second derivative (For ReLU, the second derivative is 0)
\begin{align*}
\frac{\partial^2 f(x)}{ \partial x^2 } = & ~ \left[ \sum_{j=1}^t u_j \cdot \phi'' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right) \right. \\
& ~ \cdot \sum_{i=1}^k v_{j,i} \phi'(w_i^\top \cdot x) \sum_{i'=1}^k v_{j,i'} \phi'(w_{i'}^\top x) w_i w_{i'}^\top  \\
& ~ + \sum_{j=1}^t u_j \cdot \phi' \left( \sum_{i=1}^k v_{j,i} \cdot \phi(w_i^\top \cdot x) \right)  \\
& ~ \left. \cdot \sum_{i=1}^k v_{j,i} \phi''(w_i^\top \cdot x) w_i w_i^\top   \right]
\end{align*}

\section{Sufficient condition on activation not change}

\subsection{2-layer NN}
Without loss of generality, let's look at the 1st unit (node) in the hidden layer. If $x+\delta$ has the same activation as $x$, it means that either they are both activated  
\begin{align}
	& \sum_{i=1}^{d} W_{1i} x_i + b_1 > 0 \\ 
    & \sum_{i=1}^{d} W_{1i} (x_i+\delta_i) + b_1 > 0 
\end{align}
or they are both deactivated
\begin{align}
	& \sum_{i=1}^{d} W_{1i} x_i + b_1 \leq 0 \\ 
    & \sum_{i=1}^{d} W_{1i} (x_i+\delta_i) + b_1 \leq 0. 
\end{align}
If $\delta$ satisfies the following condition, then the activation status will not change (i.e. the sufficient condition of remaining the same activation status):
\begin{equation}
 	| \sum_{i=1}^{d} W_{1i} \delta_i | < |\sum_{i=1}^{d} W_{1i} x_i + b_1 |. 
\end{equation}
Meanwhile, with H\"older's inequality, we can bound $| \sum_{i=1}^{d} W_{1i} \delta_i |$ as follows 

\begin{equation}
	| \sum_{i=1}^{d} W_{1i} \delta_i | \leq \| W_{1:} \|_q \cdot \| \delta \|_{p} , 
\end{equation}
where $1/p + 1/q = 1$, $p,q \geq 1$. Therefore, if we have 
\begin{equation}
\| W_{1:} \|_q \cdot \| \delta \|_{p} < |\sum_{i=1}^{d} W_{1i} x_i + b_1 | \Rightarrow  \| \delta \|_{p} < \frac{|\sum_{i=1}^{d} W_{1i} x_i + b_1|}{\| W_{1:} \|_q},
\end{equation}
then we can make sure $x$ and $x+\delta$ have the same activation status on the node 1 in the hidden layer. Similarly, we can derive the sufficient condition for node $j$ and the sufficient condition for all the nodes remaining the same activation status is 
\begin{equation}
\label{eq:sufficient_delta_same_act}
	\| \delta \|_{p} \leq \inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q}. 
\end{equation}

\section{Combine LP formulation with activation status}
\begin{eqnarray}
\underset{\delta}{\text{minimize  }} && \| \delta \|_p \nonumber\\
\text{subject to } && g(x_0 + \delta) < 0 \label{eq:general_opt}
\end{eqnarray}
where $g(x_0 + \delta) = f_c(x_0 + \delta) - f_j(x_0 + \delta)$ and $f(x_0 + \delta) = W^{(n)} \sigma(W^{(n-1)} \sigma(...W^{(1)}(x_0 + \delta)))$, where $W^{(n)}$ is the weight matrix of $n$th layer. The optimization formulation is exact -- if we can solve \eqref{eq:general_opt}, we get an effective attack with minimal norm. However, the constraint set in \eqref{eq:general_opt} is non-convex for general activation function.  For ReLU, the constraint set can be non-convex as well. Below, we discuss the cases where the constraint set is linear in 2-layer NN. 

\subsection{2-layer NN}
If we add the bound \eqref{eq:sufficient_delta_same_act} as an additional constraint in \eqref{eq:general_opt}, then we are guaranteed that the activation status won't change for $x_0 + \delta$ and we can directly solve the following without using the constraints in Bastani's paper:
\begin{eqnarray}
\underset{\delta}{\text{minimize  }} && \| \delta \|_p \nonumber\\
\text{subject to } &&  \sum_{r \in A(\bm{x_0})} ( \bm{V}_{cr} - \bm{V}_{jr} ) \cdot (\bm{w}_r (\bm{x}_0+\bm{\delta}) + b_r) < 0 \label{eq:lily_bastani_opt} \\
&&  \| \delta \|_{p} \leq \inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q} \nonumber 
\end{eqnarray}
If \eqref{eq:lily_bastani_opt} is feasible, then $\delta^*$ is the minimum distortion of $\bm{x}_0$ and we should get the same solution as Bastani's paper; if \eqref{eq:lily_bastani_opt} is infeasible, then $\inf_{j} \frac{|\sum_{i=1}^{d} W_{ji} x_i + b_j|}{\| W_{j:} \|_q}$ is a strict lower bound of minimum distortion (i.e. we won't over-approximate the lower bound as in the calculation in clever).   

Alternatively, we can also combine the idea of Lipschitz constant with the activation status and obtain a strict analytic lower bound for $\bm{x}_0$ (to be illustrated later)




==> _todo.tex <==
\iffalse

\section*{Writing plans and Ideas}
\subsection*{Theory}
\begin{itemize}
\item Derived gradient norm bound for n-layer network [Lily]
\item Derived required activation change bound for n-layer network [Lily]
\item Try to deal with CNN (simple 2-layer is enough)
\end{itemize}

\subsection*{Experiments}
\begin{itemize}
\item Compare with our theoretical bound with 
  \begin{itemize}
  \item adversarial distortion found by CW
  \item lower bound by CLEVER
  \item lower bound by Szegedy Lipschitz operator norm 
  \item Bastani's LP form [Hongge]
  \item Reluplex [Hongge]
  \end{itemize}
  
\item Target network: 2-4 layer ReLU MLP, possibly 2-3 layer CNN, for MNIST/Cifar
\end{itemize}

\fi







==> oldmnist_cifar_compare_adv_retrain.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on large MNIST and CIFAR models with adversarial training for three targeted attack classes.}
\label{tb:reluplex}
\scalebox{0.7}{
\begin{tabular}{cccccccc}
\cline{1-8}
                            & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network} & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{5}{*}{\makecell{MNIST\\3,1024}}     & Fast-Lin                    &         .01069            &           .01582            &        .10701             &         .02286              &      .0111                &        .03029               \\
                                              & Fast-Lip                    &         .00861            &           .00938            &        .01197             &         .01422              &      .0161                &        .01957               \\
                                              & LP                          &         .2474             &           .01677            &        .2505              &         .02409              &      .2601                &        .03181               \\
                                              & PGD                         &                           .03990&                             .08751&                           .03990&                             .12311&                           .03990&        .15653               \\ \hline

\multirow{5}{*}{\makecell{CIFAR\\5,2048}}     & Fast-Lin                    &         .01069            &           .01582            &        .10701             &         .02286              &      .0111                &        .03029               \\
                                              & Fast-Lip                    &         .00861            &           .00938            &        .01197             &         .01422              &      .0161                &        .01957               \\
                                              & LP                          &         .2474             &           .01677            &        .2505              &         .02409              &      .2601                &        .03181               \\
                                              & PGD                         &                           .07610&                             .01626&                           .07610&                             .04114&                           .07610&        .04615               \\ \hline

\end{tabular}}
\end{table}


==> oldmnist_cifar_compare_dropout.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on large MNIST and CIFAR models with dropout for three targeted attack classes.}
\label{tb:reluplex}
\scalebox{0.7}{
\begin{tabular}{cccccccc}
\cline{1-8}
                            & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network} & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{5}{*}{\makecell{MNIST\\3,1024}}     & Fast-Lin                    &         .01069            &           .01582            &        .10701             &         .02286              &      .0111                &        .03029               \\
                                              & Fast-Lip                    &         .00861            &           .00938            &        .01197             &         .01422              &      .0161                &        .01957               \\
                                              & LP                          &         .2474             &           .01677            &        .2505              &         .02409              &      .2601                &        .03181               \\
                                              & PGD                         &                           .03990&                             .08751&                           .03990&                             .12311&                           .03990&        .15653               \\ \hline

\multirow{5}{*}{\makecell{CIFAR\\5,2048}}     & Fast-Lin                    &         .01069            &           .01582            &        .10701             &         .02286              &      .0111                &        .03029               \\
                                              & Fast-Lip                    &         .00861            &           .00938            &        .01197             &         .01422              &      .0161                &        .01957               \\
                                              & LP                          &         .2474             &           .01677            &        .2505              &         .02409              &      .2601                &        .03181               \\
                                              & PGD                         &                           .07037&                             .08455&                           .07037&                             .10870&                           .07037&        .07357               \\ \hline

\end{tabular}}
\end{table}


==> oldtab_mnist_cifar_compare_dd_adv.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on large MNIST and CIFAR models with defensive distillation (temperature = 100) for three targeted attack classes.}
\label{tb:distill}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cc|ccc|ccc|ccc}
\cline{1-11}
                             & \multicolumn{1}{c|}{}       & \multicolumn{3}{c|}{runner-up}        & \multicolumn{3}{c|}{random}           & \multicolumn{3}{c}{least-likely}                     \\ \hline
\multicolumn{1}{c|}{Network} & \multicolumn{1}{c|}{Method} & Undefended &    DD    & Adv. Training & Undefended &    DD    & Adv. Training & Undefended &    DD    & Adv. Training                \\ \hline

\multirow{2}{*}{\makecell{MNIST\\3*[1024]}}     &  Fast-Lin  &          &          &          &          &          &          &          &          &          \\
                                                 &  Fast-Lip  &          &          &          &          &          &          &          &          &          \\ \hline
\multirow{2}{*}{\makecell{MNIST\\4*[1024]}}     &  Fast-Lin  &          &          &          &          &          &          &          &          &          \\ 
                                                 &  Fast-Lip  &          &          &          &          &          &          &          &          &          \\ \hline

\end{tabular}}
\end{table}



==> oldtab_mnist_cifar_compare_l1.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{EAD} on large MNIST and CIFAR models for three targeted attack classes. \textbf{LP-Full} is computationally infeasible for 100 images in the MNIST 3-layer model, so we report results on 5 images$^\dagger$. Similarly, \textbf{LP} becomes computationally infeasible for CIFAR networks so we omit their numbers. $\mathbf{L_1}$ \textbf{norm}. EAD 1000 iterations}
\label{tb:mnist_cifar_compare_l1}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\cline{1-8}
                                              & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network}                  & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{4}{*}{\makecell{MNIST\\2*[1024]}}   & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                              & Fast-Lip                    &                     &                       &                     &                       &                      &                       \\
                                              & LP                          &                     &                       &                     &                       &                      &                       \\
                                              & EAD                         &          .22322           &    9.5295                   &           .22322          &         17.259              &           .22322          &           23.933            \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{4}{*}{\makecell{MNIST\\3*[1024]}}   & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                              & Fast-Lip                    &                     &                       &                     &                       &                     &                       \\
                                              & LP                          &                     &                       &                     &                       &                     &                       \\
					      & LP-Full$^\dagger$ 		    &                  &                       &                  &                       &                  &                       \\
                                              & EAD                         &           .24123          &   10.159                    &          .24123           &       17.796                &           .24123          &              22.395         \\
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{4}{*}{\makecell{MNIST\\4*[1024]}}   & Fast-Lin                    &                      &                       &                      &                       &                      &                       \\
                                              & Fast-Lip                    &                      &                       &                       &                       &                       &                       \\
                                              & LP                          &                   &                       &                    &                       &                    &                       \\
                                              & EAD                         &            .26665         &   10.079                    &            .26665        &          17.2             &          .26665           &        23.91               \\
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\5*[2048]}}   & Fast-Lin                    &                      &                       &                      &                       &                      &                       \\
                                              & Fast-Lip                    &                     &                       &                      &                       &                      &                       \\
                                              & EAD                         &           .40441          &   7.6529                    &         .40441            &           21.643            &          .40441           &            34.497           \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\6*[2048]}}   & Fast-Lin                    &                      &                       &                    &                       &                     &                       \\
                                              & EAD                         &          .42786           &     6.0112                  &             .42786        &         17.16             &             .42786        &          28.958             \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\7*[1024]}}   & Fast-Lin                    &                     &                       &                     &                       &                    &                       \\
                                              & EAD                         &           .36170          &    7.9987                   &          .36170           &           22.18            &          .36170           &            31.529           \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\end{tabular}}
\end{table}



==> oldtab_mnist_cifar_compare_l2.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{CW} on large MNIST and CIFAR models for three targeted attack classes. \textbf{LP-Full} is computationally infeasible for 100 images in the MNIST 3-layer model, so we report results on 5 images$^\dagger$. Similarly, \textbf{LP} becomes computationally infeasible for CIFAR networks so we omit their numbers. $\mathbf{L_2}$ \textbf{norm} CW 2000 iterations}
\label{tb:mnist_cifar_compare_l2}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\cline{1-8}
                                              & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network}                  & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{4}{*}{\makecell{MNIST\\2*[1024]}}   & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                              & Fast-Lip                    &                     &                       &                     &                       &                      &                       \\
                                              & LP                          &                     &                       &                     &                       &                      &                       \\
                                              & CW                         &           .60800          &    1.1874                   &             .60800        &              1.8779         &           .60800          &          2.4556             \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{4}{*}{\makecell{MNIST\\3*[1024]}}   & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                              & Fast-Lip                    &                     &                       &                     &                       &                     &                       \\
                                              & LP                          &                     &                       &                     &                       &                     &                       \\
					      & LP-Full$^\dagger$ 		    &                  &                       &                  &                       &                  &                       \\
                                              & CW                         &           .60838          &    1.3513                   &            .53242         &             2.0387          &          .53242           &             2.4916          \\
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{4}{*}{\makecell{MNIST\\4*[1024]}}   & Fast-Lin                    &                      &                       &                      &                       &                      &                       \\
                                              & Fast-Lip                    &                      &                       &                       &                       &                       &                       \\
                                              & LP                          &                   &                       &                    &                       &                    &                       \\
                                              & CW                         &            .62657         &   1.2422                    &           .62657          &     1.8921                  &           .62657          &  2.4451                     \\
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\5*[2048]}}   & Fast-Lin                    &                      &                       &                      &                       &                      &                       \\
                                              & Fast-Lip                    &                     &                       &                      &                       &                      &                       \\
                                              & CW            &      .65675       &          .3778           &            .65675           &           .94973          &              .65675         &           1.4379                                \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline

\multirow{2}{*}{\makecell{CIFAR\\6*[2048]}}   & Fast-Lin                    &                     &                       &                     &                       &                    &                       \\
                                              & CW                         &            .67498         &      .29795                 &           .67498          &            .76347           &          .67498           &             1.2111          \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
 \multirow{2}{*}{\makecell{CIFAR\\7*[1024]}}   & Fast-Lin                    &                      &                       &                    &                       &                     &                       \\
                                              & CW                         &            .54304         &  .39426                     &          .54304           &    .97302                  &           .54304          &  1.3709                     \\ 
                                              & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline                                             
                                          
\end{tabular}}
\end{table}



==> oldtab_mnist_cifar_compare_linf.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on large MNIST and CIFAR models for three targeted attack classes. \textbf{LP-Full} is computationally infeasible for 100 images in the MNIST 3-layer model, so we report results on 5 images$^\dagger$. Similarly, \textbf{LP} becomes computationally infeasible for CIFAR networks so we omit their numbers. $\mathbf{L_\infty}$ \textbf{norm}}
\label{tb:mnist_cifar_compare_linf}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\cline{1-8}
                                              & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network}                  & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{4}{*}{\makecell{MNIST\\2*[1024]}}   & Fast-Lin                    &         .08211            &           .02249            &        .08084             &         .03073              &      .08216               &        .03835               \\
                                              & Fast-Lip                    &         .10191            &           .01797            &        .14203             &         .02515              &      .1790                &        .03128               \\
                                              & LP                          &         8.1968            &           .02487            &        8.8897             &         .03375              &      9.437                &        .04258               \\
                                              & PGD                         &         .03673            &           .07310            &        .03673             &         .11210              &      .03673               &        .14116               \\ 
                                              & CLEVER                      &                           &           .04116            &                           &         .06669              &                           &        .08632               \\ \hline
\multirow{4}{*}{\makecell{MNIST\\3*[1024]}}   & Fast-Lin                    &         .88654            &           .01826            &        1.2865             &         .02211              &      1.2887               &        .02427               \\
                                              & Fast-Lip                    &         1.2849            &           .00965            &        1.0725             &         .01217              &      1.2025               &        .01377               \\
                                              & LP                          &         20.134            &           .02008            &        21.477             &         .02422              &      22.310               &        .02658               \\
					      & LP-Full$^\dagger$ 		    &         4.04 hrs          &           .02256            &        4.14 hrs           &         .02584              &      4.09 hrs             &        .02784               \\
                                              & PGD                         &         .03990            &           .08751            &         .03990            &         .12311              &      .03990               &        .15653               \\
                                              & CLEVER                      &                           &           .04511            &                           &         .06686              &                           &        .07717               \\ \hline
\multirow{4}{*}{\makecell{MNIST\\4*[1024]}}   & Fast-Lin                    &         3.701             &           .00715            &        3.750              &         .00822              &      3.754                &        .00898               \\
                                              & Fast-Lip                    &         .5672             &           .00087            &        .737               &         .00145              &      .789                 &        .00183               \\
                                              & LP                          &         1093.8            &           .00730            &        1328.5             &         .00847              &      1068.6               &        .00932               \\
                                              & PGD                         &         .04154            &           .10853            &        .04154             &         .14635              &      .04154               &        .18066               \\
                                              & CLEVER                      &                           &           .04302            &                           &         .07055              &                           &        .09380               \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\5*[2048]}}   & Fast-Lin                    &         32.53             &           .00137            &        33.06              &         .00170              &      35.30                &        .00188               \\
                                              & Fast-Lip                    &         7.770             &           .00012            &        11.87              &         .00022              &      13.96                &        .00030               \\
                                              & PGD                         &         .07610            &           .01626            &        .07610             &         .04114              &      .07610               &        .04615               \\ 
                                              & CLEVER                      &                           &           .00614            &                           &         .01507              &                           &        .02116               \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\6*[2048]}}   & Fast-Lin                    &         49.23             &           .00075            &        50.167             &         .00090              &      52.125               &        .00095               \\
                                              & PGD                         &         .07845            &           .01122            &        .07845             &         .026066             &      .07845               &        .03556               \\ 
                                              & CLEVER                      &                           &           .00540            &                           &         .01303              &                           &        .01998               \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\7*[1024]}}   & Fast-Lin                    &         19.025            &           .00119            &        17.289             &         .00134              &      17.928               &        .00141               \\
                                              & PGD                         &         .06647            &           .01378            &        .06647             &         .03472              &      .06647               &        .05215               \\ 
                                              & CLEVER                      &                           &           .00624            &                           &         .01202              &                           &        .01510               \\ \hline
\end{tabular}}
\end{table}



==> oldtab_reluplex_compare_all_widetab.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Comparison of our proposed certified lower bounds \textbf{Fast-Lin} and \textbf{Fast-Lip}, the lower bounds found by \textbf{LP} and \textbf{LP-Full}, the lower bounds found by \textbf{CLEVER}, the exact minimum distortion found by \textbf{Reluplex}, and the upper bounds found by \textbf{Attack} algorithms (CW $\ell_\infty$ for $p = \infty$, CW $\ell_2$ for $p = 2$, EAD for $p = 1$) on 2, 3 layers toy MNIST networks with \textit{only 20 neurons per layer}. Differences of lower bounds and speedup are measured on the two corresponding bold numbers. Note that \textit{LP-full and Reluplex are very slow} and cannot scale to any practical networks, and the purpose of this table is to show how far away our fast bounds are from the true (or more accurate but very expensive) bounds.}
\label{tab:tab1-smallnetwork}
\scalebox{0.62}{
\begin{tabular}{|c|c|c|cccc||c||c||cc||cccc||c||c|}
\hline
\multicolumn{3}{|c|}{Toy Networks}                                                                                                 & \multicolumn{8}{c|}{Average Magnitude of Distortion on 100 Images}                                                                       & \multicolumn{6}{c|}{Average Running Time per Image}                                      \\ \hline
\multirow{2}{*}{Network}                                                    & \multirow{2}{*}{$p$-norm}   & \multirow{2}{*}{Target}  & \multicolumn{4}{c||}{Certified Bounds}                    & \multirow{2}{*}{difference} & Exact       & \multicolumn{2}{c|}{Uncertified} & \multicolumn{4}{c||}{Certified Bounds}                    &       Exact        & \multirow{2}{*}{Speedup}    \\ \cline{4-7}\cline{9-16}
                                                                            &                             &                          &     Fast-Lin &     Fast-Lip &     LP        &     LP-Full &                             & Reluplex    & CLEVER     & Attack              &     Fast-Lin &     Fast-Lip &      LP      &      LP-Full &      Reluplex      &                             \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ 2*{[}20{]}\end{tabular}} & \multirow{3}{*}{$p=\infty$} & top2                     & \bf 0.01904  &     0.01667  & \bf 0.01968   &     0.01968 &   3.25 \%                   & 0.04145     & 0.0235     & 0.07419             & \bf  3 ms    &      4 ms    & \bf 38 ms    &       2 s    &       134 s        & \bf  13x                       \\
                                                                            &                             & rand                     & \bf 0.03073  &     0.02699  & \bf 0.03189   &     0.03189 &   3.64 \%                   & 0.07765     & 0.0428     & 0.13034             & \bf  3 ms    &      6 ms    & \bf 42 ms    &       2 s    &       38 s         & \bf  14x                       \\
                                                                            &                             & least                    & \bf 0.04455  &     0.03976  & \bf 0.04618   &     0.04618 &   3.53 \%                   & 0.11711     & 0.0662     & 0.16967             & \bf  3 ms    &      10 ms   & \bf 45 ms    &       2 s    &       360 s        & \bf  15x                       \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=2$}      & top2                     &     0.03708  & \bf 0.21944  &     0.04204   & \bf 0.56372 &   61.07\%                   & -           & 0.4615     & 0.64669             &      3 ms    & \bf  33 ms   &      2 s     &  \bf  21 s   &       -            & \bf  636x                       \\
                                                                            &                             & rand                     &     0.05251  & \bf 0.37414  &     0.05937   & \bf 0.91816 &   59.25\%                   & -           & 0.8426     & 1.19630             &      3 ms    & \bf  43 ms   &      2 s     &  \bf  23 s   &       -            & \bf  534x                       \\
                                                                            &                             & least                    &     0.07418  & \bf 0.60673  &     0.08653   & \bf 1.34214 &   54.79\%                   & -           & 1.315      & 1.88830             &      3 ms    & \bf  51 ms   &      4 s     &  \bf  26 s   &       -            & \bf  510x                       \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=1$}      & top2                     &     0.03832  & \bf 2.11064  &     0.04322   & \bf 2.81713 &   25.08\%                   & -           & 3.168      & 5.38380             &      3 ms    & \bf  62 ms   &      2 s     &  \bf  16 s   &       -            & \bf  258x                       \\
                                                                            &                             & rand                     &     0.05387  & \bf 3.84835  &     0.06075   & \bf 4.68225 &   17.81\%                   & -           & 5.858      & 11.4760             &      3 ms    & \bf  73 ms   &      2 s     &  \bf  17 s   &       -            & \bf  233x                       \\
                                                                            &                             & least                    &     0.07598  & \bf 6.35152  &     0.08869   & \bf 6.83578 &   7.08 \%                   & -           & 9.250      & 19.5960             &      3 ms    & \bf  82 ms   &      2 s     &  \bf  18 s   &       -            & \bf  220x                       \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ 3*{[}20{]}\end{tabular}} & \multirow{3}{*}{$p=\infty$} & top2                     & \bf 0.01582  &     0.00938  &     0.01680   & \bf 0.01707 &   7.32 \%                   & 0.04234     & 0.0223     & 0.11562             &  \bf 5 ms    &       5 ms   &      478 ms  &  \bf  6 s    &       4.7 hrs      & \bf  1200x                     \\
                                                                            &                             & rand                     & \bf 0.02286  &     0.01422  &     0.02414   & \bf 0.02462 &   7.15 \%                   & 0.06824     & 0.0385     & 0.14176             &  \bf 6 ms    &       7 ms   &      564 ms  &  \bf  7 s    &       11.6 hrs     & \bf  1167x                     \\
                                                                            &                             & least                    & \bf 0.03029  &     0.01957  &     0.03194   & \bf 0.03264 &   7.20 \%                   & 0.10449     & 0.0566     & 0.18056             &  \bf 5 ms    &       9 ms   &      585 ms  &  \bf  7 s    &       12.6 hrs     & \bf  1400x                     \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=2$}      & top2                     &     0.03510  & \bf 0.08422  &     0.03906   & \bf 0.49015 &   82.82\%                   & -           & 0.4231     & 0.74117             &      6 ms    & \bf  43 ms   &      2 s     &  \bf  57 s   &       -            & \bf  1326x                     \\
                                                                            &                             & rand                     &     0.04470  & \bf 0.12876  &     0.04906   & \bf 0.70955 &   81.85\%                   & -           & 0.7331     & 1.22570             &      5 ms    & \bf  58 ms   &      2 s     &  \bf  66 s   &       -            & \bf  1138x                     \\
                                                                            &                             & least                    &     0.05642  & \bf 0.18975  &     0.06247   & \bf 0.94241 &   79.87\%                   & -           & 1.100      & 1.71090             &      5 ms    & \bf  70 ms   &      2 s     &  \bf  77 s   &       -            & \bf  1100x                     \\ \cline{2-17} 
                                                                            & \multirow{3}{*}{$p=1$}      & top2                     &     0.03653  & \bf 0.65567  &     0.04051   & \bf 2.50097 &   73.78\%                   & -           & 2.950      & 6.13750             &      5 ms    & \bf 107 ms   &      3 s     &  \bf  75 s   &       -            & \bf  701x                      \\
                                                                            &                             & rand                     &     0.04618  & \bf 1.18553  &     0.05057   & \bf 3.57400 &   66.83\%                   & -           & 4.990      & 10.7220             &      5 ms    & \bf 129 ms   &      3 s     &  \bf  82 s   &       -            & \bf  636x                      \\
                                                                            &                             & least                    &     0.05822  & \bf 1.99773  &     0.06431   & \bf 4.69673 &   57.47\%                   & -           & 7.131      & 15.6850             &      5 ms    & \bf 145 ms   &      3 s     &  \bf  86 s   &       -            & \bf  593x                      \\ \hline
\end{tabular}
}
\end{table*}


==> oldtab_reluplex_compare_l1.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the exact minimum distortion for 3 target classes found by Reluplex, and the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{EAD} on 2 and 3 layer small MNIST networks.}
\label{tb:reluplex_l1}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
%\scalebox{1}{ %%% 0.7 in ICML submission
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\cline{1-8}
                                                & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network}                    & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{5}{*}{\makecell{MNIST\\2*[20]}}       & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                                & Fast-Lip                    &                     &                       &                     &                       &                     &                       \\

                                                & LP                          &                     &                       &                      &                       &                      &                       \\
                                                & EAD                         &            .47097         &   .44178                    &          .47097           &     .52866                  &          .47097           &          .64533             \\
                                                & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{5}{*}{\makecell{MNIST\\3*[20]}}       & Fast-Lin                    &                     &                       &                     &                       &                      &                       \\
                                                & Fast-Lip                    &                     &                       &                     &                       &                      &                       \\

                                                & LP                          &                      &                       &                      &                       &                      &                       \\
		                                & LP-Full                     &                     &                       &                      &                       &                      &                       \\	
                                                & EAD                         &          .43016           &           .44238            &            .43016         &            .58324           &             .43016        &             .69461          \\
                                                & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\end{tabular}
}
\end{table}

==> oldtab_reluplex_compare_l2.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison of the exact minimum distortion for 3 target classes found by Reluplex, and the lower/upper bounds found by our proposed algorithms, and \textbf{LP} and \textbf{CW} on 2 and 3 layer small MNIST networks.}
\label{tb:reluplex_l2}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
%\scalebox{1}{ %%% 0.7 in ICML submission
% use resize box will automatically resize the table in both single and double column modes
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccc}
\cline{1-8}
                                                & \multicolumn{1}{c|}{}       & \multicolumn{2}{c|}{runner-up}                          & \multicolumn{2}{c|}{random}                             & \multicolumn{2}{c}{least-likely}                       \\ \hline
\multicolumn{1}{c|}{Network}                    & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{$\delta$} & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c}{$\delta$} \\ \hline
\multirow{5}{*}{\makecell{MNIST\\2*[20]}}       & Fast-Lin                    &                     &                       &                     &                       &                     &                       \\
                                                & Fast-Lip                    &                     &                       &                     &                       &                     &                       \\

                                                & LP                          &                     &                       &                      &                       &                      &                       \\
                                                & CW                         &             .58357        &    .64669                   &            .58357         &       1.1963                &           .58357          &       1.8883                \\
                                                & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\multirow{5}{*}{\makecell{MNIST\\3*[20]}}       & Fast-Lin                    &                     &                       &                     &                       &                      &                       \\
                                                & Fast-Lip                    &                     &                       &                     &                       &                      &                       \\

                                                & LP                          &                      &                       &                      &                       &                      &                       \\
		                                & LP-Full                     &                     &                       &                      &                       &                      &                       \\	
                                                & CW                         &           .60536          &   .74117                    &           .60536          &    1.2257                   &            .60536         &         1.7109              \\
                                                & CLEVER                      &                           &                       &                           &                       &                           &                       \\ \hline
\end{tabular}
}
\end{table}

==> tab_mnist_cifar_compare_main.tex <==
\begin{table*}[htbp]
\centering
\caption{Comparison of our proposed certified lower bounds \textbf{Fast-Lin}, \textbf{Fast-Lip} with other lower bounds (\textbf{LP}, \textbf{Op-norm}, \textbf{CLEVER}) and upper bounds (\textbf{Attack} algorithms: CW for $p = 2, \infty$, EAD for $p = 1$) on \textit{large networks} with 2-7 layers, 1024 or 2048 nodes in each layer. Differences of lower bounds and speedup are measured on the two \textbf{bold} numbers in each row. Note that \lpfull and \reluplex are \textit{computationally infeasible} for all the networks reported here. Omitted numbers (``\textbf{-}'') indicate these methods are computationally infeasible for that network. For \textbf{Op-norm}, computation time for each image is negligible as the operator norms can be pre-computed.}
\label{tb:largenetwork}
\scalebox{0.63}{
\begin{tabular}{|c|c|cc|cc||c||cc||cc|c||c|}
\hline

\multicolumn{2}{|c|}{Large Networks}                                                                        & \multicolumn{7}{c||}{Average Magnitude of Distortion on 100 Images}                                                                                                             & \multicolumn{4}{c|}{Average Running Time per Image}       \\ \hline
\multirow{3}{*}{Network}                                                      & \multirow{3}{*}{$p$}        & \multicolumn{4}{c||}{Certified Bounds}                                                     &  diff            & \multicolumn{2}{c||}{Uncertified}               & \multicolumn{3}{c||}{Certified Bounds}                   & Speedup        \\ \cline{3-6}\cline{8-12}
                                                                              &                             & \multicolumn{2}{c|}{Our bounds} &     LP                  &  Op-norm                       &  ours          & CLEVER                      & Attacks           & \multicolumn{2}{c|}{Our bounds}  &    LP                 & ours         \\ \cline{3-4}\cline{10-11}
                                                                              &                             &     Fast-Lin &   Fast-Lip       &   (Baseline)     &  \cite{szegedy2013intriguing}  &  vs. LP            & \cite{weng2017evaluating}   & CW/EAD            &     Fast-Lin      &     Fast-Lip & (Baseline)   & vs. LP           \\ \hline


\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\  $2 \times [1024]$\end{tabular}} &    $\infty$           & \bf 0.03083 & 0.02512     & \bf 0.03386 & 0.00263 & -8.9\%  & 0.0708 & 0.1291  & \bf 156 ms & 219 ms     & \bf 20.8 s & 133X  \\
                                                                                    &    $2$                & \bf 0.63299 & 0.59033     & \bf 0.75164 & 0.40201 & -15.8\% & 1.2841 & 1.8779  & \bf 128 ms & 234 ms     & \bf 195 s  & 1523X \\
                                                                                    &    $1$                & 3.88241     & \bf 5.10000 & \bf 4.47158 & 0.35957 & +14.1\% & 7.4186 & 17.259  & 139 ms     & \bf 1.40 s & \bf 48.1 s & 34X   \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\  $3 \times [1024]$\end{tabular}} &    $\infty$           & \bf 0.02216 & 0.01236     & \bf 0.02428 & 0.00007 & -8.7\%  & 0.0717 & 0.1484  & \bf 1.12 s & 1.11 s     & \bf 52.7 s & 47X   \\
                                                                                    &    $2$                & \bf 0.43892 & 0.26980     & \bf 0.49715 & 0.10233 & -11.7\% & 1.2441 & 2.0387  & \bf 906 ms & 914 ms     & \bf 714 s  & 788X  \\
                                                                                    &    $1$                & \bf 2.59898 & 2.25950     & \bf 2.91766 & 0.01133 & -10.9\% & 7.2177 & 17.796  & \bf 863 ms & 3.84 s     & \bf 109 s  & 126X  \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\  $4 \times [1024]$\end{tabular}} &    $\infty$           & \bf 0.00823 & 0.00264     & -           & 0.00001 & -       & 0.0793 & 0.1303  & \bf 2.25 s & 3.08 s     & -          & -     \\
                                                                                    &    $2$                & \bf 0.18891 & 0.06487     & -           & 0.17734 & -       & 1.4231 & 1.8921  & \bf 2.37 s & 2.72 s     & -          & -     \\
                                                                                    &    $1$                & \bf 1.57649 & 0.72800     & -           & 0.00183 & -       & 8.9764 & 17.200  & \bf 2.42 s & 2.91 s     & -          & -     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR\\  $5 \times [2048]$\end{tabular}} &    $\infty$           & \bf 0.00170 & 0.00030     & -           & 0.00000 & -       & 0.0147 & 0.02351 & \bf 26.2 s & 78.1 s     & -          & -     \\
                                                                                    &    $2$                & \bf 0.07654 & 0.01417     & -           & 0.00333 & -       & 0.6399 & 0.9497  & \bf 36.8 s & 49.4 s     & -          & -     \\
                                                                                    &    $1$                & \bf 1.18928 & 0.31984     & -           & 0.00000 & -       & 9.7145 & 21.643  & \bf 37.5 s & 53.6 s     & -          & -     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR\\  $6 \times [2048]$\end{tabular}} &    $\infty$           & \bf 0.00090 & 0.00007     & -           & 0.00000 & -       & 0.0131 & 0.01866 & \bf 37.0 s & 119 s      & -          & -     \\
                                                                                    &    $2$                & \bf 0.04129 & 0.00331     & -           & 0.01079 & -       & 0.5860 & 0.7635  & \bf 60.2 s & 95.6 s     & -          & -     \\
                                                                                    &    $1$                & \bf 0.72178 & 0.08212     & -           & 0.00000 & -       & 8.2507 & 17.160  & \bf 61.4 s & 88.2 s     & -          & -     \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}CIFAR\\  $7 \times [1024]$\end{tabular}} &    $\infty$           & \bf 0.00134 & 0.00008     & -           & 0.00000 & -       & 0.0112 & 0.0218  & \bf 10.6 s & 29.2 s     & -          & -     \\
                                                                                    &    $2$                & \bf 0.05938 & 0.00407     & -           & 0.00029 & -       & 0.5145 & 0.9730  & \bf 16.9 s & 27.3 s     & -          & -     \\
                                                                                    &    $1$                & \bf 0.86467 & 0.09239     & -           & 0.00000 & -       & 8.630  & 22.180  & \bf 17.6 s & 26.7 s     & -          & -     \\ \hline
 \end{tabular}
}
\end{table*}


==> tab_reluplex_compare_app_timeonly.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htbp]
\centering
\caption{Comparison of our proposed certified lower bounds \textbf{Fast-Lin} and \textbf{Fast-Lip}, the lower bounds found by \textbf{LP} and \textbf{LP-Full}, the lower bounds found by \textbf{CLEVER}, the exact minimum distortion found by \textbf{Reluplex}, and the upper bounds found by \textbf{Attack} algorithms (CW $\ell_\infty$ for $p = \infty$, CW $\ell_2$ for $p = 2$, and EAD for $p = 1$) on 2, 3 layers toy MNIST networks with \textit{only 20 neurons per layer}. Differences of lower bounds and speedup are measured on the two corresponding \textbf{bold} numbers in each row, representing the best answer from our proposed algorithms and LP based approaches. Reluplex is designed to verify $\ell_\infty$ robustness so we omit its numbers for $\ell_2$ and $\ell_1$. Note that \textit{LP-full and Reluplex are very slow} and cannot scale to any practical networks, and the purpose of this table is to show how close our fast bounds are compared to the true minimum distortion provided by \textbf{Reluplex} and the bounds that are slightly tighter but very expensive (e.g. \textbf{LP-Full}).}
\label{tb:smallnetwork_app}
\centering
\scalebox{0.76}{
\begin{tabular}{|c|c|c|
>{\centering\arraybackslash}p{9ex}
>{\centering\arraybackslash}p{9ex}|
>{\centering\arraybackslash}p{9ex}
>{\centering\arraybackslash}p{9ex}
||c||c|}
\hline
\multicolumn{3}{|c|}{Toy Networks}                                                                                                     & \multicolumn{6}{c|}{Average Running Time per Image}                                                             \\ \hline
\multirow{3}{*}{Network}                                                       & \multirow{2}{*}{$p$}        & \multirow{3}{*}{Target} & \multicolumn{4}{c||}{Certified Bounds}                                      &       Exact     & Speedup         \\ \cline{4-8}
                                                                               &                             &                         & \multicolumn{2}{c|}{Our bounds} & \multicolumn{2}{c||}{Baselines} &    Reluplex     & ours vs.       \\ \cline{4-7}

                                                                               &                             &           & Fast-Lin    & Fast-Lip    & LP         & LP-Full    & \cite{katz2017reluplex} &    LP-(full)     \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ $2\times[20]$\end{tabular}} & \multirow{3}{*}{$\infty$}   & runner-up & \bf 3.09 ms & 3.49 ms     & \bf 217 ms & 1.74 s     & 134 s    & 70X    \\
                                                                               &                             & rand      & \bf 3.25 ms & 5.53 ms     & \bf 234 ms & 1.93 s     & 38 s     & 72X    \\
                                                                               &                             & least     & \bf 3.37 ms & 8.90 ms     & \bf 250 ms & 1.97 s     & 360 s    & 74X    \\ \cline{2-9}
                                                                               & \multirow{3}{*}{$2$}        & runner-up & \bf 3.00 ms & 3.76 ms     & 1.10 s     & \bf 20.6 s & -        & 6864X  \\
                                                                               &                             & rand      & \bf 3.37 ms & 6.16 ms     & 1.20 s     & \bf 23.1 s & -        & 6838X  \\
                                                                               &                             & least     & \bf 3.29 ms & 9.89 ms     & 1.27 s     & \bf 26.4 s & -        & 8021X  \\ \cline{2-9}
                                                                               & \multirow{3}{*}{$1$}        & runner-up & 2.85 ms     & \bf 39.2 ms & 1.27 s     & \bf 16.1 s & -        & 412X   \\
                                                                               &                             & rand      & 3.32 ms     & \bf 54.8 ms & 1.59 s     & \bf 17.3 s & -        & 316X   \\
                                                                               &                             & least     & 3.46 ms     & \bf 68.1 ms & 1.74 s     & \bf 17.7 s & -        & 260X   \\ \hline
\multirow{9}{*}{\begin{tabular}[c]{@{}c@{}}MNIST\\ $3\times[20]$\end{tabular}} & \multirow{3}{*}{$\infty$}   & runner-up & \bf 5.58 ms & 3.64 ms     & 253 ms     & \bf 6.12 s & 4.7 hrs  & 1096X  \\
                                                                               &                             & rand      & \bf 6.12 ms & 5.23 ms     & 291 ms     & \bf 7.16 s & 11.6 hrs & 1171X  \\
                                                                               &                             & least     & \bf 6.62 ms & 7.06 ms     & 307 ms     & \bf 7.30 s & 12.6 hrs & 1102X  \\ \cline{2-9}
                                                                               & \multirow{3}{*}{$2$}        & runner-up & \bf 5.35 ms & 3.95 ms     & 1.22 s     & \bf 57.5 s & -        & 10742X \\
                                                                               &                             & rand      & \bf 5.86 ms & 5.81 ms     & 1.27 s     & \bf 66.3 s & -        & 11325X \\
                                                                               &                             & least     & \bf 5.94 ms & 7.55 ms     & 1.34 s     & \bf 77.3 s & -        & 13016X \\ \cline{2-9}
                                                                               & \multirow{3}{*}{$1$}        & runner-up & \bf 5.45 ms & 39.6 ms     & 1.27 s     & \bf 75.0 s & -        & 13763X \\
                                                                               &                             & rand      & \bf 5.56 ms & 52.9 ms     & 1.47 s     & \bf 82.0 s & -        & 14742X \\
                                                                               &                             & least     & 6.07 ms     & \bf 65.9 ms & 1.68 s     & \bf 85.9 s & -        & 1304X  \\ \hline
\end{tabular}
}
\end{table*}


==> tab_untargeted.tex <==

% new table (updated: 03.27) with p = inf, 2, 1
% tab_untargeted_all.tex
\begin{table}[htbp]
\centering
\caption{Comparison of the lower/upper bounds of minimum distortion found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on MNIST and CIFAR datasets for \textit{untargeted} attacks}
\label{tb:untargeted}
\ifdef{\useicmlformat}
{
}{
\vspace{3mm} %%% added by zhao, otherwise it looks ugly
}
\scalebox{0.65}{%%% 0.8 in ICML submission
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{c|}{untargeted robustness}                               & \multicolumn{2}{c}{$p=\infty$}               & \multicolumn{2}{|c}{$p=2$}               & \multicolumn{2}{|c}{$p=1$}              \\ \hline
\multicolumn{1}{c|}{Model}                 & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c}{Time}  & $\delta$  	& \multicolumn{1}{|c}{Time} & $\delta$     & \multicolumn{1}{|c}{Time} & $\delta$    \\ \hline
\multirow{4}{*}{\makecell{MNIST\\3*[1024]}}& Fast-Lin                    &      1.3279               &  0.01805  	&     1.0255                &  0.02530     &     1.0308                &  0.00257    \\
                                           & Fast-Lip                    &      0.2307               &  0.00092  	&     3.8982                &  0.04137     &     19.012                &  0.15820     \\
                                           & LP                          &      65.08                &  0.01980  	&     number                &  number      &     number                &  number     \\
                                           & PGD                  &      .14082		     &  .12291  	&     .14082                &  2.2637     &     .14082                &  44.99     \\ 
 & CW                  &      .54333		     &  .20905  	&     .54333                &  1.118      &     .54333                &  16.372     \\ 
 & EAD                  &      .23190		     &  .56182  	&     .23190                &  1.5429      &     .23190                &  9.0044     \\ \hline
\multirow{2}{*}{\makecell{CIFAR\\5*[2048]}}& Fast-Lin                    &      30.39                &  0.00084  	&     58.66                 &  0.00137     &     58.21                 &  0.00139    \\
                                           & PGD                  &      .42190              &  .0052734  	&     .42190                &  .27581      &     .42190                &  14.894     \\ 
                                           & CW                  &      .65393		     &  .017015 	&     .65393                &  .23201      &     .65393                &  10.051     \\ 
                                           & EAD                  &      .48805		     &  .15248  	&     .48805                &  .50908     &     .48805                &  4.6307     \\ \hline
\end{tabular}
}
\end{table}



%% Table in the submission
% \begin{table}[htbp]
% \centering
% \caption{Comparison of the lower/upper bounds of minimum distortion found by our proposed algorithms, and \textbf{LP} and \textbf{PGD} on MNIST and CIFAR datasets for \textit{untargeted} attacks}
% \label{tb:untargeted}
% \ifdef{\useicmlformat}
% {
% }{
% \vspace{3mm} %%% added by zhao, otherwise it looks ugly
% }
% \scalebox{1}{%%% 0.8 in ICML submission
% \begin{tabular}{cccc}
% \hline
%                                            & \multicolumn{1}{c|}{}       & \multicolumn{2}{c}{untargeted}      \\ \hline
% \multicolumn{1}{c|}{Model}                 & \multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{Time} & $\delta$ \\ \hline
% \multirow{4}{*}{\makecell{MNIST\\3*[1024]}} & Fast-Lin                   &      1.3279               &  0.01805 \\
%                                            & Fast-Lip                    &      0.2307               &  0.00092 \\
%                                            & LP                          &      65.08                &  0.01980 \\
%                                            & PGD                         &                     0.4461&          0.12654\\ \hline
% \multirow{2}{*}{\makecell{CIFAR\\5*[2048]}}& Fast-Lin                    &      30.39                &  0.00084   \\
%                                            & PGD                         &                     .08354&          0.00522\\ \hline
% \end{tabular}
% }
% \end{table}


==> trash.tex <==
\begin{comment}
\iffalse
\textcolor{blue}{Hongge: I changed the claims a little bit\\
\begin{claim}
If there exists a set-cover $C \subseteq [d]$ with $\cup_{j\in C} S_j = [n]$ and $|C| \leq r$, then there exists a point $y \in [0,1]^d$ such that $\| x - y \|_1 \leq r$ and $F(y) > 0$.
\begin{proof}
Without loss of generality, let the set cover to be $\{S_1,S_2,...,S_r\}$. Let $y_1=y_2=...=y_r=1$ and $y_{r+1}=y_{r+2}=...=y_{d}=0.$ So we have $t_1=t_2=...=t_r=\delta$ and $v_1=v_2=...=v_n=\delta$, since $\{S_1,S_2,...,S_r\}$ is a set cover. Then $F(y)=w=\min_iv_i=\delta>0.$ Note we also have $|y|=r.$
\end{proof}
\end{claim}
\begin{claim}
If for every $C \subseteq [d]$ with $\cup_{j \in C}S_j = U$ satisfies that $|C| \geq r+1  $, then for all $y\in [0,1]^d$ satisfies that $\| x - y\|_1 \leq  r $, $F(y) \leq 0$ holds.
\begin{proof}
Proof by contradiction. We assume there exists $y$ such that $F(y)> 0$ and $\| y\|_1 \leq  r .$ $$F(y)> 0\Rightarrow \forall i,\ v_i>0\Rightarrow\forall i,\ \exists j(i)\in T_i,\ s.t.\ t_j>0\Rightarrow\forall i,\ \exists j(i)\in T_i,\ s.t.\ 1-\delta<y_{j(i)}\leq 1.$$Since $\sum_{j\in[d]}|y_j|\leq  r $, we have
$$\sum_{k\in\{j(i)|i\in[n]\}}|y_k|\leq\sum_{j\in[d]}|y_j|\leq r .$$
Because for all $k\in\{j(i)|i\in[n]\}$, $|y_k|>1-\delta=1-1/d$, we have $$|\{j(i)|i\in[n]\}|\leq \frac{ r }{(1-1/d)}< r+1$$ when $d$ is large enough. So $\{j(i)|i\in[n]\}$ is a set cover with size less than $r+1$. Contradiction.
\end{proof}
\end{claim}
Using Claim A.14 and Claim A.15 we have
\begin{claim}
For any SET-COVER problem, there exists a set-cover $C \subseteq [d]$ with $\cup_{j\in C} S_j = [n]$ and $|C| \leq r$ if and only if  there exists a point $y \in [0,1]^d$ such that $\| x - y \|_1 \leq r$ and $F(y) > 0$.
\end{claim}
}


\textcolor{blue}{
Hongge: If you agree with my suggestion above, I think there actually exists an easier construction. \begin{align*}
\phi_{1,j} =
\begin{cases}
1 & \text{~if~} u_j \geq 1, \\
0 & \text{~otherwise~}.
\end{cases}
\end{align*}
\begin{align*}
\phi_{2,i} =
\begin{cases}
1, & \text{~if~} \sum_{j\in T_i} u_j \geq 1,\\
0, & \text{~otherwise}.
\end{cases}
\end{align*}
For final output node $w$, we define an activation function $\psi$ satisfies that
\begin{align*}
\psi = 
\begin{cases}
1, & \text{~if~} \sum_{i=1}^n v_i \geq n, \\
0, & \text{~otherwise}.
\end{cases}
\end{align*}
Then we have
$$F(y)=1\iff \forall i\in[n],\exists j(i)\in T_i\text{~such that~}y_{j(i)}\geq 1$$
$$F(y)=0\iff \exists i\in[n],\forall j\in T_i,y_j< 1$$
So if there exists $|y|_1\leq r$ such that $F(x)=1$, we have $$\sum_{k\in\{j(i)|i\in[n]\}}y_k\leq\sum_{k\in[d]}y_k\leq r.$$But $y_{j(i)}\geq 1$, so $|\{j(i)|i\in[n]\}|\leq r,$ which means SET-COVER of size at most $r$ exists. Conversely, if SET-COVER of size at most $r$ exists, we simply set those used sets' $y_j$ as 1 and others as 0. Then $|y|\leq r$ and $F(y)=1.$ This means that 
$$\exists\text{~SET-COVER with size at most }r\iff\exists |y|_1\leq r, F(y)=1.$$So solving ROBUST-NET(R) is at least as hard as solving SET-COVER. But the arbitrary activation function assumption may be too strong. \\Can we do a proof with only ReLU activation? the thing is that here we use the property of incontinuity. if it is relu, it may be hard to prove. but i believe we can still do it by using relu with very large coefficients to approximate the step function.
}
\fi
\end{comment}

%\textcolor{red}{Huan: I will check your claims and proof.  I remember there are reasons that we need to use the $\delta$ trick. For example, 
%if $(1.0, 0, 0, 0)$ ($r=1$) is an adversarial example using the construction above, $(1.0, 0.9999, 0.9999, 0.9999)$ is also an adversarial example, but with $r$ close to 4. Then you cannot tell if the set cover has 1, 2, or 3 sets. Using the $\delta$ trick, it will guarantee that the largest point you can find is $(1.0, \delta, \delta, \delta)$ with $r=1+3\delta$, $r$ is an estimate close enough to the true cover number with bounded error.}

\begin{comment}
\iffalse
\textcolor{red}{Huan: All the activation functions above can be implemented combining linear layers and ReLUs. For example, $\max(t_1, t_2) = \max(t_1 - t_2, 0) + t_2$. (We probably can write a few propositions for them). If you found anything that cannot be implemented, let me know. Thanks!}\\
\textcolor{blue}{Hongge: Using linear and ReLU can only generate continuous activation functions. But step function is not continuous and so as to some of our activations in Theorem A.11 using step function. These implementations work in discrete scenario as in Theorem A.8 but do not work in Theorem A.11. For example, the $\psi$ in Theorem A.11. \begin{align*}
\psi = 
\begin{cases}
1, & \text{~if~} \sum_{i=1}^n v_i \geq n(1-\delta), \\
0, & \text{~otherwise}.
\end{cases}
\end{align*}
When $\sum_{i=1}^n v_i =n(1-\delta)/2$ you should have $\psi=0$. But if you use the ReLU+linear implementation 
\begin{align*}
\psi = 1 - \max \left( 0, 1 - \frac{1}{n(1-\delta)}\sum_{i=1}^n v_i \right)
\end{align*}you will get $\psi=0.5$. 
So this implementation is actually NOT correct. Similarly for $\phi_{1,j}$ and $\phi_{1,j}$, they are not continuous, so they CANNOT be implemented by ReLU+linear. They can only be approximated by ReLU+linear.}
\fi

\end{comment}
